Multimodal Manoeuvre and Trajectory Prediction for Automated Driving on Highways Using Transformer Networks

Predicting the behaviour (i.e., manoeuvre/trajectory) of other road users, including vehicles, is critical for the safe and efficient operation of autonomous vehicles (AVs), a.k.a., automated driving systems (ADSs). Due to the uncertain future behaviour of vehicles, multiple future behaviour modes are often plausible for a vehicle in a given driving scene. Therefore, multimodal prediction can provide richer information than single-mode prediction, enabling AVs to perform a better risk assessment. To this end, we propose a novel multimodal prediction framework that can predict multiple plausible behaviour modes and their likelihoods. The proposed framework includes a bespoke problem formulation for manoeuvre prediction, a novel transformer-based prediction model, and a tailored training method for multimodal manoeuvre and trajectory prediction. The performance of the framework is evaluated using three public highway driving datasets, namely NGSIM, highD, and exiD. The results show that our framework outperforms the state-of-the-art multimodal methods in terms of prediction error and is capable of predicting plausible manoeuvre and trajectory modes.

==> deletions.tex <==
Given a local coordinate system with an x-axis in direction of travel and a y-axis from right to left (as depicted in Fig.~\ref{intro_fig}), a consecutive series of locations on a trajectory are classified as $RLC$ if the vehicle at one point crosses the right lane marking and continuously has negative gradient before and after crossing. Similarly, a consecutive series of locations are classified as $LLC$ if the vehicle at one point crosses the left lane marking and continuously has a positive gradient before and after crossing. A waypoint that is neither classified as $LLC$ nor $RLC$ is considered as $LK$. Therefore, lateral displacements that do not lead to or follow a lane crossing are considered as $LK$ manoeuvre.


\begin{table}[]
\centering
\caption{List of selected input features categorised based on their contribution to representation of a driving scene$^a$}
\label{tab:feature_list}
\begin{tabular}{@{}cl@{}}
\toprule
Type                                                                                  & \multicolumn{1}{c}{Features}                                                                              \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TV \\ Dynamics\end{tabular}}               & (1) Longitudinal acceleration of TV                                                                       \\
                                                                                      & (2) Lateral distance of TV to   the left lane marking                                                     \\
                                                                                      & (3) Lateral acceleration of   the prediction target                                                       \\ \midrule
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Interaction\\  with   SVs$^b$\end{tabular}} & (4) Longitudinal distance of TV   to PV,                                                                  \\
                                                                                      & (5) Longitudinal distance of   TV to RPV                                                                  \\
                                                                                      & (6) Longitudinal distance of TV to FV                                                                     \\
                                                                                      & (7) Lateral distance of TV to RV                                                                          \\
                                                                                      & (8) Lateral distance of TV to RFV                                                                         \\
                                                                                      & (9)   Relative longitudinal velocity of TV w.r.t. PV                                                      \\
                                                                                      & (10)   Relative longitudinal velocity of TV w.r.t. FV                                                     \\
                                                                                      & (11) Relative lateral velocity   of TV w.r.t. PV                                                          \\
                                                                                      & (12)   Relative lateral velocity of TV w.r.t. RPV                                                         \\
                                                                                      & (13)   Relative lateral velocity of TV w.r.t. RV                                                          \\
                                                                                      & (14)   Relative lateral velocity of TV w.r.t. LV                                                          \\
                                                                                      & \begin{tabular}[c]{@{}l@{}}(15)   Relative longitudinal acceleration of TV \\      w.r.t RPV\end{tabular} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Environment\\  Context\end{tabular}}       & (16) Existence of left lane                                                                               \\
                                                                                      & (17) Existence of right lane                                                                              \\
                                                                                      & (18) lane width                                                                                           \\ \bottomrule
\end{tabular}
\footnotesize{$^a$TV: Target Vehicle, SV: Surrounding Vehicle, PV: Preceding Vehicle, RPV: Right Preceding Vehicle, RV: Right Vehicle, RFV: Right Following Vehicle, FV: Following Vehicle, LV: Left Vehicle, $^b$ In case of non-existance of a surrounding vehicle, longitudinal distances are set to 400 meters, lateral distances are set to 3 times the lane width, and relative velocities and accelerations are set to 0.
}\\

\end{table}

\begin{figure}[!t]
\centering
\includegraphics[width=3.4in]{Figures/Manoeuvre_Prediction.pdf}
\caption{Multimodal manoeuvre prediction outputs.}
\label{fig:man_outputs}
\end{figure}

